Multi-view Inference for Relation Extraction with Uncertain Knowledge

Knowledge graphs (KGs) are widely used to facilitate relation extraction (RE) tasks. While most previous RE methods focus on leveraging deterministic KGs, uncertain KGs, which assign a confidence score for each relation instance, can provide prior probability distributions of relational facts as valuable external knowledge for RE models. This paper proposes to exploit uncertain knowledge to improve relation extraction. Specifically, we introduce ProBase, an uncertain KG that indicates to what extent a target entity belongs to a concept, into our RE architecture. We then design a novel multi-view inference framework to systematically integrate local context and global knowledge across three views: mention-, entity- and concept-view. The experimental results show that our model achieves competitive performances on both sentence- and document-level relation extraction, which verifies the effectiveness of introducing uncertain knowledge and the multi-view inference framework that we design.

==> 1-introduction.tex <==
\section{Introduction}

The main goal of relation extraction is to classify the semantic relationship between entities under a given context. It has plenty of practical applications, such as dialogue systems \cite{DBLP:conf/aaai/YoungCCZBH18}, question answering \cite{DBLP:conf/acl/YuYHSXZ17} and information retrieval \cite{DBLP:conf/sigir/KadryD17}.

Most of the previous work focus on designing advanced neural networks \cite{DBLP:conf/aaai/HeCLZZZ18,DBLP:conf/acl/GuoZL19,DBLP:conf/acl/YeLXSCZ19,DBLP:conf/acl/SahuCMA19,DBLP:conf/aaai/GuptaRSR19}, ignoring the rich information existing in knowledge graphs (KGs). KGs contain various prior knowledge, and provide the relationship between two entities or the relatedness among entities and concepts. The external knowledge can improve the model's generalization ability and facilitate the performance of relation extraction \cite{DBLP:conf/akbc/VergaM16,DBLP:journals/eswa/LiM19}. In general, KGs are categorized into two types \cite{DBLP:conf/aaai/ChenCSSZ19}: 1) Deterministic KGs, such as FreeBase \cite{DBLP:conf/sigmod/BollackerEPST08}, contain  deterministic relationship between entities; 2) Uncertain KGs, such as ConceptNet \cite{DBLP:conf/aaai/SpeerCH17} and ProBase \cite{DBLP:conf/sigmod/WuLWZ12}. For given two words (typically two entities or an entity and a concept) and a relationship, uncertain KG provides a confidence score that measures the possibility of the two words have the given relation. 
\begin{figure}[h]
    \centering
    \includegraphics[width=1.\linewidth]{intro}
    \caption{An example of a three-view inference framework for document-level relation extraction. In document-level relation extraction, an entity may contain various mentions, usually with different forms. For a given entity, the local interactive representation is aggregated by different mention representations through mention2Entity-view. This is a cross-view process between mention- and entity-view. Moreover, by retrieving uncertain KG, the concepts and weighting scores are used to produce the concept representation, which will gather descriptions of entities and concepts to obtain global interactive representations. This is a cross-view procedure between entity- and concept-view. Finally, entity-view is used for final information aggregation and relation extraction. Sentence-level relation extraction just contains entity- and concept-view. The figure is better viewed in color.}
    \label{intro}
\end{figure}
%A gated mechanism is employed to combine the local- and global entity representations for final prediction at entity-view.

The majority of the studies on relation extraction with KGs \cite{DBLP:conf/akbc/VergaM16,DBLP:conf/coling/LeiCLDY0S18,DBLP:conf/naacl/XuB19} focus on distant supervision relation extraction (DSRE) \cite{DBLP:conf/acl/MintzBSJ09}. Since the datasets used in DSRE are labeled by different KGs automatically and suffer from the wrong-labeling problem, it is a natural way that leveraging KGs to facilitate the performance. However, due to the annotation setting, DSRE only uses deterministic KGs. Meanwhile, the relations in those datasets must be a subset of the predefined relations in deterministic KGs \cite{DBLP:conf/acl/MintzBSJ09,DBLP:conf/naacl/XuB19}, which limits the application in the practical scenario.  

In the supervised relation extraction, adding the information about which concepts the target entity belongs to is beneficial for the model's performance, but there are few works leverage KGs for external knowledge. Although some researchers use BERT \cite{DBLP:conf/naacl/DevlinCLT19} to encode the input context, which provides rich semantic information, \cite{DBLP:journals/corr/abs-1911-03024,DBLP:conf/emnlp/PetersNLSJSS19} point out that the performance of a pre-trained language model can still be improved by incorporating external knowledge. In most cases, for a given entity, only the most likely (the top-K) concepts that the entity belongs to are needed when building a relation extraction model, using too many related concepts will negatively influence the performance (\textbf{Section 5.2}). However, the deterministic KGs only provide the relational triples, and models cannot select the most related concepts through prior knowledge. By contrast, uncertain KGs further provide the confidence score for each relational triple. Thus the model can use the top-K concepts as supplementary information to facilitate the performance. Meanwhile, the confidence scores provide a prior probability distribution of concepts for an entity, which gives critical information when the contextual information is insufficient. Since lots of predefined relationships in deterministic KGs and ConceptNet are not matching the relation types in supervised relation extraction datasets (such as ACE2005\footnote{https://catalog.ldc.upenn.edu/ldc2006t06} and DocRED \cite{DBLP:conf/acl/YaoYLHLLLHZS19}). ProBase just provides the \textit{IsA} relation between an entity and a concept, which indicates if the target entity belongs to the concept. It is convenient for us to couple with supervised relation extraction datasets, therefore we use ProBase to retrieve the related concepts for an entity. Besides, the text descriptions of entities and concepts can be found on Wikipedia, these descriptions provide rich semantic information for relation extraction, but they are ignored by most of the existing methods. Hence we retrieve the text descriptions from Wikipedia to enrich the representations of entities and concepts, and build a new corpus that couples with ProBase, named ProBase\_Desp, more details about the construction of ProBase\_Desp can be found in the supplementary materials. 

Moreover, as the input context contains the local entity representation with internal semantic features, ProBase and ProBase\_Desp provide the global entity representation with the external knowledge. To obtain discriminative feature vectors, it is non-trivial to aggregate the local and global information effectively. For different representation levels from various resources, inspired by \cite{DBLP:conf/kdd/HaoCYSW19}, we design a multi-view inference framework that can better aggregate information by cross-view inference. For sentence-level relation extraction, we use a two-view inference framework containing entity- and concept-view representations. For document-level relation extraction, a three-view inference framework is designed that further adding mention-view representation. So the multi-view framework can handle both sentence- and document-level relation extraction tasks.

In this paper, we propose a novel framework named UNKMI, which incorporates \textbf{UN}certain \textbf{K}nowledge and \textbf{M}ulti-view \textbf{I}nference for supervised relation extraction. Unlike previous models that learn prior knowledge using binary relation fact labels from KGs, UNKMI characterizes relation facts by the confidence scores of uncertain knowledge, as shown in Figure \ref{intro}. Specifically, for a given entity, UNKMI first retrieves the top-K concepts that the target entity most likely belongs to, then leverages a multi-view inference framework to aggregate the local and global information, attention and gate mechanisms are also employed to extract the most discriminative information. Experimental results show that UNKMI achieves promising results and consistently outperforms state-of-the-art models on sentence- and document-level relation extraction tasks. In summary, our main contributions are as follows:
\begin{itemize}
     \item We propose a new model named UNKMI, this is the first study that leverages uncertain knowledge and text descriptions as well as a multi-view inference framework for relation extraction. UNKMI can effectively combine local and global representations.
    \item We conduct various experiments and achieve the state-of-the-art results on both sentence- and document-level relation extraction tasks, detailed analyses about UNKMI are also presented.
    \item We will release the ProBase\_Desp for further research, which contains more than 15,000,000 entity and concept descriptions retrieved from Wikipedia. We believe ProBase\_Desp can be utilized by the majority of the natural language processing and multi-modal tasks. 
\end{itemize}

%Besides, UNKMI trains the relation extraction module and uncertain KG jointly. The uncertain KG trained using TransE \cite{DBLP:conf/nips/BordesUGWY13}, and the embeddings of entities and concepts in uncertain KG are initialized by encoding the ProBase\_Desp using BERT, instead of randomly initialized in most of the previous work.

%The confidence scores mainly come from the co-occurrence frequency in the huge number of web pages.


